Fair Decision Making using Privacy-Protected Data

Data collected about individuals is regularly used to make decisions that impact those same individuals. We consider settings where sensitive personal data is used to decide who will receive resources or benefits. While it is well known that there is a tradeoff between protecting privacy and the accuracy of decisions, we initiate a first-of-its-kind study into the impact of formally private mechanisms (based on differential privacy) on fair and equitable decision-making. We empirically investigate novel tradeoffs on two real-world decisions made using U.S. Census data (allocation of federal funds and assignment of voting rights benefits) as well as a classic apportionment problem. Our results show that if decisions are made using an $\epsilon$-differentially private version of the data, under strict privacy constraints (smaller $\epsilon$), the noise added to achieve privacy may disproportionately impact some groups over others. We propose novel measures of fairness in the context of randomized differentially private algorithms and identify a range of causes of outcome disparities.

==> findings.tex <==
\section{Preliminary Findings}
Possible findings which could be supported by simple empirical studies:

\subsection{Equal noise can have unequal impacts}

Even a carefully-designed privacy mechanism, which enforces equal noise for each population, can have unequal impacts when standard allocation methods are used. 

\begin{outline}[enumerate]
\1 For threshold allocation problems, equal noise disproportionately impacts populations close to the threshold.
\1 For Huntington-Hill apportionment, equal noise in population totals disproportionately impacts some states. 
\end{outline}


\subsection{Common privacy mechanisms create disparate impacts}
There are a number of examples of commonly-used (or even state-of-the-art) privacy mechanisms that lead to one or more of the disparate impacts identified above. 

\paragraph{Unequal expected loss}

\begin{outline}[enumerate]
\1 Identity on county population counts leads to unequal noise (no bias)
\1 Hierarchical counts on county, state, nation with LS inference leads to unequal noise (no bias)
\1 DAWA or MWEM: unequal noise, bias
\end{outline}

\paragraph{Bias}
\begin{outline}[enumerate]
\1 DAWA or MWEM: unequal noise and bias
\end{outline}


\section{Remedies: resolving disparate impacts}

\paragraph{Trade-off in existing mechanisms}
It is possible to design unbiased mechanisms, which offer equal noise to populations.  But there appears to be a cost to doing so: total error is increased, consistency may be impossible...

\begin{outline}
\1 Matrix-mechanism approaches: measure trade-offs between "fair" strategies in terms of accuracy
\1 DAWA is best algorithm in some cases, but it is biased.  measure cost of using next best "fair" alternative?
\end{outline}







==> formalizing.tex <==
\section{Formalizing allocation problems}

\subsection{Setup}
The allocation problems above can be formalized as assignments to a set of geographic units, as follows:

\begin{outline}[itemize]

\1 Populations, $P={p_1 \dots p_n}$ (often defined by geographic units such as states, counties, school districts)

\1 Sensitive variables, $V$: properties of some $p_i$, which can be described by queries, e.g:  we write $V[p_i]$ for a set of queries evaluated on the population $p_i$ and resulting in values for the variables. Queries might include:

	\2 Count[*]($p_i$)
	\2 Count[$age>18$]($p_i$)


\1 Outcome space, O: set of possible outcomes (e.g. non-negative dollar values, seats in apportionment allocation, binary allocations in above examples)

\1 Allocation formula: a function $F: G \rightarrow O$ assigns an outcome to each geographic unit, expressed in terms of the variables.  
	
\end{outline}
	
Then we can define the true allocation and the private allocation:


\begin{outline}
	
\1 {\bf True allocation:}  F is computed for each $p_i$ using true values of sensitive variables for $p_i$: $F(V[p_i])$

\1 {\bf Private allocation:} $F$ is computed for each $p_i$ using noisy private values of sensitive variables for $p_i$. $F(\tilde{V}[p_i])$ where $\tilde{V}$ indicates the noisy variable values. 
\end{outline}


\subsection{Forms of allocation functions}

\begin{outline}
\1 Population proportional: 
\1 Threshold
\1 Threshold proportional
\1 Apportionment	
\end{outline}




==> impact.tex <==
\section{Impacts}

Below we describe various impacts that may arise when allocation is performed on privacy-protected data.  We begin by noting that, even using true statistics, certain allocations treat populations differently:

{\bf Inherent inequity} It is not always possible to treat all populations equally, particularly when the resource is indivisible. A classic example is apportionment of representatives, which requires the division of a fixed number of representatives among the states. 

\subsection{Potential impacts of noise}
\begin{outline}[enumerate]
	
\1[E0] {\bf Unequal loss}  Because privacy protection algorithms are randomized, any given run of the algorithm will result in unequal loss for different populations.  This impact may be unavoidable for randomized privacy mechanisms, but may imply long-lasting negative impacts for some populations, especially when allocations happen infrequently (e.g. decennially).

\1[E1] {\bf Unequal expected loss}	Although loss may be unequal for any particular run of an allocation mechanism, we may hope that over the long run, that is, in expectation (over the randomness of the privacy algorithm), loss is equal.  A population with higher expected loss is disadvantaged, relative to the true allocation.

\1[E2] {\bf Biased loss}	Even when the expected loss of two populations is equal, it remains possible that the noise distribution is biased in a manner that disadvantages one population. 

\1[E4] {\bf Population non-monotonicity}
When populations grow, recipients expect allocations to increase or remain unchanged.  In the presence of noise, this may not hold.  A variant of this compares the allocations to two populations where one has grown faster than the other, with the expectation that the faster-growing population receives a larger allocation.

\1[E5] {\bf Allocation non-monotonicity}
When the supply of the allocated resource grows (more funding, or more representatives in the House), recipients expect their allocation to increase or stay the same.  In the presence of noise, this may not hold in general.  In the context of apportionment, the so-called ``Alabama paradox'' involved apportionment algorithms in which an increased number of total house seats led to a lower apportionment for Alabama.  Current algorithms avoid this paradox. 

\1[E3] {\bf Unequal expected loss for multiple allocations}
When we consider multiple allocation problems, supported by a set of private statistics about populations, we may desire that expected loss (averaged over populations) be equal for each allocation problem.  This would ensure, for example, that expected loss of school funding allocations is equivalent to that of low-income housing allocation.


\end{outline}

